QAID: Question Answering Inspired Few-shot Intent Detection

Intent detection with semantically similar fine-grained intents is a challenging task. To address it, we reformulate intent detection as a question-answering retrieval task by treating utterances and intent names as questions and answers. To that end, we utilize a question-answering retrieval architecture and adopt a two stages training schema with batch contrastive loss. In the pre-training stage, we improve query representations through self-supervised training. Then, in the fine-tuning stage, we increase contextualized token-level similarity scores between queries and answers from the same intent. Our results on three few-shot intent detection benchmarks achieve state-of-the-art performance.

==> chapters/6-ablation.tex <==
\section{Ablation Tests}
%--------  Contribution to a plain classifier ---------------------
\begin{table}[h]\centering
\begin{tabular}{lcccccc}
\toprule 
\multirow{2}{*}{Model} & \multicolumn{2}{c}{CLINC150} & \multicolumn{2}{c}{BANKING77} & \multicolumn{2}{c}{HWU64}\\
\cmidrule(l){2-3} \cmidrule(l){4-5} \cmidrule(l){6-7}
 & 5 & 10 & 5 & 10 & 5 & 10\\
\midrule
\textbf{Classifier results}\\
RoBerta Classifier (baseline) & 87.68 & 91.22 & 74.46 & 83.79 & 73.52 & 82.62 \\
Adding intent name as example & 89.47 & 91.91 & 78.33 & 84.93 & 79.13 & 84.69\\
initializing classification head with the intent & 72.82 & 81.89 & 63.0 & 74.86 & 51.65 & 57.65\\
Classifer+init from intents - freeze & 80.76 & 87.72 & 66.21 & 80.68 & 62.04 & 75.31\\
Classifer+init intents st-model-freeze & 88.47 & 90.78 & 76.15 & 85.61 & 68.37 & 78.31\\
Classifer - token level  & 85.71 & 90.71 & 73.33 & 83.83 & 74.98 & 83.66\\
\midrule
% \textbf{Match-Qq results}\\
% %ColBERT-Qa (Asaf) & 82.03 & 88.10 & 72.71 & 79.25 & 74.98 & 81.78 \\
% DNNC   & 91.02 & 93.76 & 80.40 & 86.71 & 80.46 & 84.72 \\
% ColBERT-Qq (Roberta-base, PT, ours) & 91.53 & 94.29 & 83.93 & 87.86 & 84.20 & 86.62 \\
% ColBert-Qq with answer as example & \boaz{Missing}\\
% ColBert-Qq with answer as another example (6/11)& \boaz{Missing}\\
% \midrule
% \textbf{Match-Qa results}\\
% ColBERT-Qa (Roberta-base, PT, ours)  & 88.44 & 93.44 & 78.73 & 86.40 & 82.82 & 86.52 \\ 
% ColBERT-Qa (Asaf - roberta-base) & 82.03 & 88.1 & 72.71 & 79.25 & 74.98 & 81.78\\
% ColBert-Qa with example as answer& \boaz{Missing}\\
% ColBert-Qa with another example as answer (6/11)& \boaz{Missing}\\
% \midrule
% \textbf{Match-Qqa results}\\
% ColBert-Both with example as answer& \boaz{Missing}\\
% ColBert-Both with example as answer (6/11 total)& \boaz{Missing}\\
% ColBERT-Both (Roberta-base, PT, ours)  & 91.73 & 94.40 & 83.20 & 87.63 & 85.22 & 87.22 \\
% QAID (Roberta-base, PT, ours) & 92.94 & 94.57 & 85.35 & 88.63 & 84.89 & 87.70\\
% QAID with example as answer& \boaz{Missing}\\
% QAID with example as answer (6/11 total)& \boaz{Missing}\\
% QAID six-datasets & 93.41 & 94.64 & 85.25 & 88.83 & 85.52 & 87.98\\
\midrule
\textbf{The contribution of batch contrastive}\\
ColBERT-Vanila (w/o PT) & 82.03 & 88.1 & 72.71 & 79.25 & 74.98 & 81.78\\
ColBERT-Vanila (with PT) & \boaz{Missing}\\
ColBERT-Vanila (with augmentation) & \boaz{Missing}\\
% ColBERT-Both (Roberta-base, PT, ours)  & 91.73 & 94.40 & 83.20 & 87.63 & 85.22 & 87.22 \\
QAID (PT) & 92.94 & 94.57 & 85.35 & 88.63 & 84.89 & 87.70\\
\midrule
\textbf{Trying different intent name options}\\
QAID new-names - with prep & 87.84 & 92.25 & 77.49 & 83.6 & 76.58 & 83.57\\
QAID new-names - bert-key & 87.53 & 92.23 & 78.62 & 85.51 & 74.49 & 84.32\\
QAID new-names - no prep & 87.41 & 91.94 & 78.1 & 83.31 & 76.49 & 85.07\\
% QAID with query and intent name & 87.61 & 91.67 & 76.74 & 84.02 & 78.19 & 84.23\\
%QAID CASE\_1\_DEL\_RANDOM\_EXAMPLE (e_{1-4}, a) & \boaz{Missing}\\
% CASE\_2\_DEL\_RANDOM\_EXAMPLE\_TO\_BE\_ANSWER
QAID (e_{1-4}, e_5) & \boaz{Missing}\\
% QAID CASE\_3\_ADD\_RANDOM\_EXAMPLE\_TO\_BE\_ANSWER
QAID (e_{1-5}, e_6) & \boaz{Missing}\\
\midrule
\textbf{Comparing cls with token level}\\
Clasifier with token level similarity & 85.71 & 90.71 & 73.33 & 83.83 & 74.98 & 81.78\\
QAID- CLS- roberta-base w/o PT & 90.52 & 93.26 & 81.61 & 86.2 & 80.45 & 86.48\\
\midrule
\textbf{Results without pretraining}\\
QAID- CLS- roberta-base w/o PT & 90.52 & 93.26 & 81.61 & 86.2 & 80.45 & 86.48\\
QAID - roberta-base w/o PT & 90.79 & 93.66 & 82.16 & 87.17 & 81.68 & 86.01\\
\midrule
QAID-Bert &  \boaz{Missing}\\
\bottomrule
\end{tabular}
\caption{
Experimental results. 
}
\label{tbl:abl-all}
\end{table}

